Enhancing Mass Customization Manufacturing: Multiobjective Metaheuristic Algorithms for flow shop Production in Smart Industry

The current landscape of massive production industries is undergoing significant transformations driven by emerging customer trends and new smart manufacturing technologies. One such change is the imperative to implement mass customization, wherein products are tailored to individual customer specifications while still ensuring cost efficiency through large-scale production processes. These shifts can profoundly impact various facets of the industry. This study focuses on the necessary adaptations in shop-floor production planning. Specifically, it proposes the use of efficient evolutionary algorithms to tackle the flowshop with missing operations, considering different optimization objectives: makespan, weighted total tardiness, and total completion time. An extensive computational experimentation is conducted across a range of realistic instances, encompassing varying numbers of jobs, operations, and probabilities of missing operations. The findings demonstrate the competitiveness of the proposed approach and enable the identification of the most suitable evolutionary algorithms for addressing this problem. Additionally, the impact of the probability of missing operations on optimization objectives is discussed.

==> material_saved.tex <==

\subsection{Mass customization impact on the shop-floor operations}

As aforementioned, an important aspect of smart industry is mass customization. Mass customization refers to the capacity of efficiently producing goods and services that are tailored to meet individual customer preferences and requirements, while still achieving economies of scale similar to mass production~\cite{baranauskas2020mapping}. Several companies have successfully invested in enhancing their mass customization strategies to offer personalized products to their customers. One example is
Nike, which allows customers to design their own sneakers through its Nike By You  platform, where they can choose colors, materials, and customize various design elements~\cite{nikeExample}. Another example is Dell, which offers customized computers and laptops through its website, allowing customers to select hardware specifications, software options, and even design their own laptop skins~\cite{dellExample}. Larger products also have entered to this wave of customization. For example in cars production, BMW enables customers to personalize their luxury vehicles with a wide range of custom features, including paint colors, interior materials, and technology options~\cite{BMWExample}. Similarly, Tesla allows customers to personalize various aspects of their electric vehicles, including battery range, interior features, and autopilot capabilities~\cite{teslaExample}. 

In this regard, mass customization has a huge impact in shop-floor operations~\cite{zawadzki2016smart}. Among the aspects that are involved in an efficient shop-floor management are: 
i) Workflow flexibility: shop floors must be designed to accommodate varying product configurations and customization options. Flexible layouts, modular workstations, and adaptable production lines are essential to seamlessly transition between different customization processes~\cite{keddis2015modeling}. In this sense, quick changeover processes, e.g., Single-Minute Exchange of Die (SMED), are crucial to transition between different customization options efficiently minimizing downtime during changes.
ii) Real-time data integration: mass customization relies on real-time data from various sources, such as customer orders, inventory levels, and production progress. Shop-floor operations need to integrate data systems to ensure accurate and up-to-date information for decision-making. Technology based on RFID devices is an ally in this sense~\cite{zhong2013rfid}. 
iii) Agile production planning: traditional batch production planning may not align with the requirements of mass customization. Agile production planning methods, such as lean manufacturing or just-in-time principles, become more relevant to optimize resources and minimize waste~\cite{ding2023combining};
iv) Inventory management: mass customization demands a delicate balance between maintaining a diverse inventory of components and minimizing excess stock. Inventory management systems must be optimized to ensure that the right components are available for each customization option~\cite{guo2018inventory};
v) Advanced manufacturing technologies: Mass customization often leverages advanced technologies like robotics, automation, and additive manufacturing. These technologies enhance efficiency, precision, and speed in producing customized products on the shop floor~\cite{savolainen2020additive};
vi) Quality 4.0: the varying processes that emerge with diverse customization options, enforce quality control to adapt to ensure consistent quality across all product variations. Thus, robust quality assurance protocols and testing procedures are crucial to maintain customer satisfaction~\cite{zonnenshain2020quality};
vii) Skilled Workforce: Shop-floor operators need to be skilled in handling various customization processes, technologies, and equipment. Training programs are essential to empower workers with the knowledge needed to execute customization tasks effectively~\cite{liboni2019smart};
viii) Smart production planning and control: aims to intelligently perform the activities of loading, scheduling, sequencing, monitoring, and controlling the use of resources and materials during production by means of data analytics, AI, and machine learning~\cite{oluyisola2022designing}.

\subsection{Related work}
The study of missing operation in regular flow shop problems (i.e., a single machine per stage) is not a new problem, it has been studied for more than two decades \cite{glass1999two}. However, in the last years it has gained renewed attention in the scientific community since, as it was mentioned previously, there is a growing tendency in the transformation of traditional manufacturing processes towards personalized manufacturing processes. \cite{dios2018efficient}. As for instance, the case of concrete personalized industry where the production process is configured as a flow shop with missing operation. In \cite{smutnicki2022cyclic}, the objective is to  minimize the cycle time, and for this, the authors developed a comprehensive innovative approach that overcomes the particular restrictions the production process has, like lags between operations. Other type of problem is tackled at \cite{ramezanian2017milp}, where a non-permutation flow shop problem with missing operation is considered. Mathematical programming models are developed to optimize the makespan in this work. Also a non-permutation flow shop problem is analyzed at \cite{rossit2021solving}, but in this case total tardiness is considered as objective function and metaheuristics are used for optimization. More recently in \cite{han2022scheduling} a missing operation flow shop problem arises at the semiconductor industry. At this case, a special feature of the studied problem is the presence of time waiting constraints, and the objective function is the minimization of total tardiness. For solving the problem heuristic algorithm are implemented. Regarding multi-objective optimization with missing operation in regular flow shop problems, the literature is more scarce. Basically, as far as the authors know, it can be found only \cite{rossit2021explicit} and \cite{rossit2022multi}, where in these works a bi-objective problem is approached by means of Evolutionary algorithms. In those studies makespan and total tardiness are minimized, and different levels of missing operations are considered.

Therefore, after revising the literature, it has not been detected  a missing operation problem with three objectives, even less that analyzed makespan, total tardiness and total completion time simultaneously. These objectives involves different relevant interests for decision makers, whom must to cope with in their optimization processes. Makespan contribute to optimizing production resources usage, reducing the idle time of them. Meanwhile, total tardiness focus on service level to the client, trying to accomplish the due dates agreed with the client. And, total completion time, try to reduce the time a production order is on the system, that is, tries to reduce the time this order is considered as work-in-progress. The present article addresses these three objectives in a multi-objective manner.
